Reinterpreting the puzzling properties of z>6 galaxies within a variable IMF framework

Recent results form the James Webb Space Telescope (JWST) report space densities for bright and massive galaxies at z>7 that far exceed expectations of theoretical models of galaxy formation, prompting a revision of our understanding of the physical processes leading to the assembly of the first luminous structures. In this work we present predictions from a realization of the GAlaxy Evolution and Assembly (GAEA) model, which implements a prescription for a variable stellar initial mass function (IMF). This prescription is inspired by high-resolution numerical simulations that account for the role of cosmic rays (CR) as regulators of the star formation rate (SFR) in giant molecular clouds. In our approach, SFR density is assumed to be a proxy for the CR density, providing a link between the IMF shape and the predicted physical conditions of the star forming interstellar medium. Our results show that, in our model framework, assuming such a variable IMF reproduces several properties of the z>6 galaxy population, with no further modification of the feedback model, including their UV luminosity functions up to z~13. In order to compare model predictions with available estimates for the galaxy stellar mass function (GSMF), we reconstruct stellar masses from the model's synthetic photometry assuming a universal IMF, reflecting standard observational practice. Under this approach, we show that the model can reproduce the evolution of the GSMF up to the highest redshifts accessible. Our findings highlight the need to consider a variable IMF shape in the error budget associated with stellar mass estimates. We show that the evolution of both the slope and normalization of the gas-phase mass metallicity relation can be used as powerful discriminant between models of early galaxy formation assuming different IMF evolution.

==> journal.tex <==
%%%%%%%%% Bibliography and bibfile
\def\aj{AJ}%
         % Astronomical Journal
\def\araa{ARA\&A}%
         % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
         % Astrophysical Journal
\def\apjl{ApJ}%
         % Astrophysical Journal, Letters
\def\apjs{ApJS}%
         % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
         % Applied Optics
\def\apss{Ap\&SS}%
         % Astrophysics and Space Science
\def\aap{A\&A}%
         % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
         % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
         % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
         % Astronomicheskii Zhurnal
\def\baas{BAAS}%
         % Bulletin of the AAS
\def\jrasc{JRASC}%
         % Journal of the RAS of Canada
\def\memras{MmRAS}%
         % Memoirs of the RAS
\def\mnras{MNRAS}%
         % Monthly Notices of the RAS
\def\pra{Phys.~Rev.~A}%
         % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
         % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
         % Physical Review C
\def\prd{Phys.~Rev.~D}%
         % Physical Review D
\def\pre{Phys.~Rev.~E}%
         % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
         % Physical Review Letters
\def\pasp{PASP}%
         % Publications of the ASP
\def\pasj{PASJ}%
         % Publications of the ASJ
\def\qjras{QJRAS}%
         % Quarterly Journal of the RAS
\def\skytel{S\&T}%
         % Sky and Telescope
\def\solphys{Sol.~Phys.}%
         % Solar Physics
\def\sovast{Soviet~Ast.}%
         % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
         % Space Science Reviews
\def\zap{ZAp}%
         % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
         % Nature
\def\iaucirc{IAU~Circ.}%
         % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
         % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
         % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
         % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
         % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
         % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
         % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
         % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
         % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
         % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
         % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
         % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
         % Physics Reports
\def\physscr{Phys.~Scr}%
         % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
         % Planetary Space Science
\def\procspie{Proc.~SPIE}%
         % Proceedings of the SPIE
\def\nar{NewAR}%
         % New Astronomy Review?
\def\na{NewA}%
         % New Astronomy ?
\def\jcap{JCAP}%
         % Journal of Cosmology and Astroparticle Physics?
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

